Optimal Control of 1D Semilinear Heat Equations with Moment-SOS Relaxations

We use moment-SOS (Sum Of Squares) relaxations to address the optimal control problem of the 1D heat equation perturbed with a nonlinear term. We extend the current framework of moment-based optimal control of PDEs to consider a quadratic cost on the control. We develop a new method to extract a nonlinear controller from approximate moments of the solution. The control law acts on the boundary of the domain and depends on the solution over the whole domain. Our method is validated numerically and compared to a linear-quadratic controller.

==> images/tikz/method_diagram.tex <==
\begin{figure}[h]
\centering
\resizebox{1\columnwidth}{0.8\height}{%
%\resizebox{0.49\textwidth}{0.82\height}{%
%\resizebox{0.49\textwidth}{!}{%

\begin{tikzpicture}[node distance=1cm, auto]
 
% Sum shape
\node[draw,
    fill=Rhodamine!50,
    minimum width=2cm,
    minimum height=1.2cm,
    text width=3cm,
    align=center
] (sum) at (0,0) {Initial nonlinear PDE.};
 
 
% Controller
\node [draw,
    fill=Goldenrod,
    minimum width=2cm,
    minimum height=1.2cm,
    text width=3cm,
    align=center,
    right=1cm of sum
]  (controller) {Write the weak formulation into GloptiPoly.};
 
% System H(s)
\node [draw,
    fill=SpringGreen, 
    minimum width=2cm, 
    minimum height=1.2cm,
    text width=3cm,
    align=center,
    right=1cm of controller
] (system) {GloptiPoly assembles the matrices of the SDP.};
 
% Sensor block
\node [draw,
    fill=SeaGreen, 
    minimum width=2cm, 
    minimum height=1.2cm,
    text width=3cm,
    align=center,
    below = 1cm of system
]  (sensor) {Solve the SDP with the solver MOSEK.};


% Numerical Simulation block
\node [draw,
    fill=SkyBlue!50, 
    minimum width=2cm, 
    minimum height=1.2cm,
    text width=3cm,
    align=center,
    left = 1cm of sensor
]  (numsim) {Extract a polynomial control law $u$ from the moments.};

% End Block
\node [draw,
    fill=Turquoise, 
    minimum width=2cm, 
    minimum height=1.2cm,
    text width=3cm,
    align=center,
    left = 1cm of numsim
]  (endblock) {Simulate numerically the PDE.};

% Dashed rectangle around the specified blocks
\node[draw, dashed, inner sep=0.5cm, fit=(controller) (system) (sensor) (numsim), label=above:{Moment overlay}] {};

% Arrows with text label
\draw[-stealth] (sum.east) -- (controller.west);
%    node[midway,above]{$e$};
 
\draw[-stealth] (controller.east) -- (system.west);
%    node[midway,above]{$u$};
    
\draw (system.east) -- ++(1,0) node[anchor=mid](output){};
 
\draw[-stealth] (output.mid) |- (sensor.east);

\draw[-stealth] (sensor.west) -- (numsim.east);

\draw[-stealth] (numsim.west) -- (endblock.east);

%\draw[-stealth] (numsim.west) -- ++(-1,0) node[anchor=mid](end){};
 
%\draw[-stealth] (numsim.west) -| (sum.south) 
%    node[near end,left]{$y_m$};
 
%\draw[stealth-] (sum.west) -- ++(-1,0) ;
%\draw[-stealth] (endblock.west) -- ++(-1,0) ;
%    node[midway,above]{$y_{ref}$};
 
\end{tikzpicture}

}
\caption{Moment-based approach for the control of PDEs.}
\label{fig:steps_extract_controller}
\end{figure}%
